On Pattern Setups and Pattern Multistructures

Modern order and lattice theory provides convenient mathematical tools for pattern mining, in particular for condensed irredundant representations of pattern spaces and their efficient generation. Formal Concept Analysis (FCA) offers a generic framework , called pattern structures, to formalize many types of patterns, such as itemsets, intervals, graph and sequence sets. Moreover, FCA provides generic algorithms to generate irredundantly all closed patterns, the only condition being that the pattern space is a meet-semilattice. This does not always hold, e.g., for sequential and graph patterns. Here, we discuss pattern setups consisting of descriptions making just a partial order. Such a framework can be too broad, causing several problems, so we propose a new model, dubbed pattern multistructure, lying between pattern setups and pattern structures, which relies on multilattices. Finally, we consider some techniques , namely completions, transforming pattern setups to pattern structures using sets/antichains of patterns.

==> AlgoPatSetup.tex <==
%\usepackage{caption}

\theoremstyle{plain}% Theorem-like structures provided by amsthm.sty
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{problem}[theorem]{Problem}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{note}{Note}
\newtheorem{question}{Question}


\newcommand{\multistructure}[0]{{multistructure}}
\newcommand{\Multistructure}[0]{{Multistructure}}
\newcommand{\multisemilattice}[0]{{multisemilattice}}
\newcommand{\meetmultisemilattice}[0]{{meet-\multisemilattice}}
\newcommand{\joinmultisemilattice}[0]{{join-\multisemilattice}}
\newcommand{\multilattice}[0]{{multilattice}}
\newcommand{\meetsemilattice}[0]{{$\wedge$-semilattice}}
\newcommand{\joinsemilattice}[0]{{$\vee$-semilattice}}
\newcommand{\minf}[0]{{\text{minf}}} % TODO Maybe change notations
\newcommand{\msup}[0]{{\text{msup}}}
\newcommand{\naturals}[1]{[#1]}
\newcommand{\figref}[1]{Fig.~\ref{#1}}


\newcommand{\cbo}[0]{{\texttt{CbO}}}
\newcommand{\jump}[0]{{\texttt{Jump}}}
\newcommand{\cboLong}[0]{{Close-by-One}}
\newcommand{\cbon}[0]{{\texttt{CbOa}}}
\newcommand{\cbonLong}[0]{{Close-by-One adapted}}
\newcommand{\seek}[0]{{\texttt{Seer}}}
\newcommand{\seekLong}[0]{{Pattern setup extents enumerator}}
\newcommand{\hunt}[0]{{\texttt{Hunt}}}
\newcommand{\grow}[0]{{\texttt{Grow}}}

\newcommand{\todoaimene}[1]{\textcolor{red}{\textbf{Aimene TODO.} #1}}
\newcommand{\todosergei}[1]{\textcolor{blue}{\textbf{Sergei TODO.} #1}}
\newcommand{\todomehdi}[1]{\textcolor{green}{\textbf{Mehdi TODO.} #1}}
\newcommand{\hfunction}[5]{\begin{aligned}
#1\::\:& #2 & \longrightarrow\:&\:#3 \\
    & #4 & \longmapsto\:&\:#5 \end{aligned}}
\newcommand{\lfunction}[5]{#1 : #2 \to #3 , #4 \mapsto #5}


\newcommand{\empha}[1]{\textbf{#1}}

\newcommand{\minimalhandle}[0]{minimal-handle}
\newcommand{\maximalhandle}[0]{maximal-handle}
\newcommand{\minimumhandle}[0]{minimum-handle}
\newcommand{\maximumhandle}[0]{maximum-handle}


\setlist{noitemsep,topsep=1pt}


\author{
\name{Aimene Belfodil\textsuperscript{a, c}\thanks{Contact Aimene Belfodil. Email: aimene.belfodil@insa-lyon.fr}, Sergei O. Kuznetsov\textsuperscript{b}, Mehdi Kaytoue\textsuperscript{a, d}}
\affil{\textsuperscript{a}Univ Lyon, INSA Lyon, CNRS, LIRIS UMR 5205, F-69621, LYON, France; \textsuperscript{b}National Research University Higher School of Economics, Moscow, Russia; \textsuperscript{c}Mobile Devices Ing{\'{e}}nierie, 100 Avenue Stalingrad, 94800, Villejuif, France; \textsuperscript{d}Infologic, 99 avenue de Lyon, 26500 Bourg-L\`es-Valence, France;}
}

\title{On Computing with Pattern Setups}


%
\begin{document}

\maketitle

\input{sections/abstract}
\input{sections/introduction}
\input{sections/preliminaries}
\input{sections/patternSetups}
\input{sections/patternStructures}
\input{sections/fromClosedToSupportClosedDescriptions.tex}
\input{sections/multilattices.tex}
\input{sections/patternMultiStructures}
\input{sections/completion}
\input{sections/conclusion}

%\newpage
\bibliographystyle{tfcad}
\bibliography{biblio}   % name your BibTeX data base

%\newpage
%\appendix
%\input{sections/proofs}
%\input{sections/multilatticemisconceptions}
%\input{sections/antichaincompletions}
\end{document}


==> figures/completejoinmultilattice.tex <==
\begin{tikzpicture}[scale=.7]
\node (a) at (-1,7) {$a$};
\node (b) at (1,7) {$b$};
\node (inf) at (0,6) {$\vdots$};
\node (cn) at (0,5) {$c_n$};
\node (ci) at (0,3.5) {$\vdots$};
\node (c1) at (0,2) {$c_1$};
\node (c0) at (0,0.5) {$c_0$};
\draw (a) -- (inf) -- (cn) -- (ci) -- (c1) -- (c0);
\draw (b) -- (inf);
\end{tikzpicture}

==> figures/completemeetmultilattice.tex <==
\begin{tikzpicture}[scale=.7]
\node (a) at (-0.5,-1) {$a$};
\node (b) at (0.5,-1) {$b$};
\node (inf) at (0,0.5) {$\vdots$};
\node (cn) at (0,2) {$c_n$};
\node (ci) at (0,3.5) {$\vdots$};
\node (c1) at (0,5) {$c_1$};
\node (c0) at (0,6) {$c_0$};
\draw (a) -- (inf) -- (cn) -- (ci) -- (c1) -- (c0);
\draw (b) -- (inf);
\end{tikzpicture}

==> figures/hassediagramdefinablesetsitemset.tex <==
\begin{tikzpicture}[scale=.7]
\node (1) at (0,-1) {$\{g_1\}$};
\node (123) at (-1.4,0.5) {$\{g_1, g_2, g_3\}$};
\node (14) at (1.4,0.5) {$\{g_1, g_4\}$};
\node (1234) at (0,2) {$\{g_1,g_2,g_3,g_4\}$};
\draw (1) -- (123) -- (1234) -- (14) -- (1);
\end{tikzpicture}

==> proofs/proof11.tex <==
\begin{proof}
Since every subsets of $\delta[A]$ has a meet then $\delta[G]$ has a meet. Thus $cov(\mathcal{G}) \neq \emptyset$. Indeed, it contains at least one element which is $\bigsqcap \delta[G]$. We conclude that all subsets $A \subseteq \mathcal{G}$ are coverables since $cov(A) \supseteq cov(\mathcal{G}) \neq \emptyset$.
\end{proof}

==> proofs/proof4.tex <==
\begin{proof} Recall that for $p \in P$ we have:
\begin{eqnarray*}
\phi_E(p) & = & \bigwedge \{e \in E \mid p \leq e\}
\end{eqnarray*}
Below, the proof of the three properties:
\begin{itemize}
\item $\phi_E$ \emph{is extensive.} This property is trivial since $p \in \{e \in E \mid p \leq e\}^\ell$ and the meet is the greatest element. Thus: $p \leq \phi_E(p)$.
\item $\phi_E$ \emph{is monotone.} let $p_1 \leq p_2$ be two elements in $P$. It is clear that: 
\begin{eqnarray*}
\{e \in E \mid p_2 \leq e\} & \subseteq & \{e \in E \mid p_1 \leq e\} \\
\{e \in E \mid p_1 \leq e\}^\ell & \subseteq & \{e \in E \mid p_2 \leq e\}^\ell
\end{eqnarray*}
Thus $\phi_E(p_1) \leq \phi_E(p_2)$. Since the maximum of the first is below the maximum of the second.
\item $\phi_E$ \emph{is idempotent.} In fact we have:
\begin{eqnarray*}
\{e \in E \mid \phi_E(p) \leq e\} & = & \{e \in E \mid p \leq e\}
\end{eqnarray*}
Inclusion $\subseteq$ is verified since $p \leq \phi_E(p)$. The second inclusion $\supseteq$ comes from the definition. Indeed, since $\phi_E(p)$ is a lower bound for $\{e \in E \mid p \leq e\}$, then for any $e \in E$ such that $p \leq e$ we have $\phi_E(p) \leq e$.

We conclude the idempotence:
\begin{eqnarray*}
\phi_E(\phi_E(p)) = \bigwedge \{e \in E \mid \phi_E(p) \leq e\} = \bigwedge \{e \in E \mid p \leq e\} = \phi_E(p)
\end{eqnarray*}
\end{itemize}

Let us show now that $\phi_E[L] = \{\bigwedge S \mid S \subseteq E\}$ by double inclusion:
\begin{itemize}
    \item[($\subseteq$)] Let be an element $c \in \phi_E[L]$, that is $\exists p \in L$ such that $c = \phi_E(p)$. Hence $\exists S \subseteq E$ such that $c = \bigwedge S$. Thus $c \in \{\bigwedge S \mid S \subseteq E\}$. 
    \item[($\supseteq$)] We have $\forall e \in E$, $\phi_E(e) = e$. Thus $E \subseteq \phi_E[L]$. Since $(\phi_E[L], \leq)$ is a meet-structure (i.e. closure system), we have: $\forall A \subseteq \phi_E[L]$, $\bigwedge A \in \phi_E[L]$. Particularly, for all $S \subseteq E$, we have $\bigwedge S \in \phi_E[L]$. We conclude that  $\{\bigwedge S \mid S \subseteq E\} \subseteq \phi_E[L]$. 
\end{itemize}
\end{proof}

==> sections/antichaincompletions.tex <==
\newpage
\section{On Antichain Completion}
A completion is a way to include (embed) a poset into another using what is called an order embedding. 

\begin{definition}[\textbf{Completion}]
Let be $(P, \leq)$ be a poset. A poset $(Q, \leqq)$ is said to be a \emph{completion} of $(P, \leq)$ if there exists an order embedding linking $(P, \leq)$ to $(Q, \leqq)$. That is a mapping $\phi : P \to Q$ s.t. $(\forall x, y \in P)$ $x \leq y \Leftrightarrow \phi(x) \leqq \phi(y)$.
\end{definition}

Different natural completion exist in the literature. For instance, the Dedekind-MacNeille completion of an arbitrary poset $(P, \leq)$ is the complete lattice $(DM(P), \subseteq)$ with $DM(P) = \{A^\ell \mid A \subseteq P\}$. The embedding is given by $\phi : P \to DM(P), x \to x^\ell$. While the Dedekind-MacNeille completion associates always a complete lattice to a poset, a completion is not necessarily always a complete lattice. We discuss here the antichain completion (see~\cite{BoldiVigna2016,crampton2001completion}).

\begin{definition}[\textbf{Antichain completion}]
Let $(P, \leq)$ be a poset, we call antichain completion of $(P, \leq)$ the poset $(\mathscr{A}(P), \leqq)$ defined as follow:
\begin{itemize}
\item The set $\mathscr{A}(P)$ denotes the set of all antichains of $(P, \leq)$.
\item The order $\leqq$ is given by: $(\forall A, B \in \mathscr{A}(P))$ $A \leqq B \Leftrightarrow \downarrow A \subseteq \downarrow B$.
\end{itemize}

In fact, there is an order embedding $\phi$ from $(P, \leq)$ to $(\mathscr{A}(P), \leqq)$ given by:
\begin{eqnarray*}
\phi : (P, \leq) \hookrightarrow (\mathscr{A}(P), \leqq), a \mapsto \{a\} 
\end{eqnarray*}
\end{definition}

Surprisingly, one can show that the antichain completion of some complete lattice can be even not a meet-semilattice. Figure \ref{fig:completelatticenotgoodantichaincompletion} depicts the Hasse diagram of a complete lattice. However, the antichain completion of such a lattice is not even a lattice. Indeed, for the antichains $A = \{a_i \mid i \in \mathbb{N}\}$ and $B = \{b_i \mid i \in \mathbb{N}\}$, we have $\downarrow A \bigcap \downarrow B = \{c_i \mid i \in \mathbb{N}\}$, however, there is no antichain $D \in \mathscr{A}(P)$ such that $\{c_i \mid i \in \mathbb{N}\} =  \downarrow D$ (see the necessary and sufficient condition formulated in \cite{BoldiVigna2016} in order to $(\mathscr{A}(P), \leqq)$ be a meet-semilattice) making the antichain completion not a meet-semilattice. \todoaimene{Reduce the size of this section and maybe show that if the antichain completion is a complete lattice (or something like that) then the embedded poset is a complete multilattice (or something like that)}


\begin{figure}[h!]
\centering
\scalebox{.9}{\input{figures/completelatticenotgoodantichaincompletion.tex}}
\caption{The Antichain completion of this complete lattice is not even a meet-semilattice  \label{fig:completelatticenotgoodantichaincompletion}}
\end{figure}



==> sections/multilatticemisconceptions.tex <==
\newpage
\section{More details about Multilattices \label{appendix:multilatticemisconception}}

In the following part of this section, we discuss here some possible misconceptions that someone could have when he he wants to generalizes quickly the concepts inherited from lattices to the more general notion of multilattices.

\subsection{Complete semimultilattices are not necessarily multilattices}
Unlike lattices where complete meet-semilattices (or complete join-semilattices) are by definition complete lattices,  not all complete meet-semimultilattice are complete join-semimultilattices and \emph{vice-versa}. This can be even worse, since a complete-semimultilattice can be even not a join-semimultilattice. Figure \ref{fig:problemincompletemsupminf} shows the Hasse-diagram of a complete meet-semimultilattice $(P, \leq)$ that is even not a join-semimultilattice. Indeed, one can show that for any arbitrary subset (including the empty set) $S \subseteq P$ we have 
$S^\ell = \downarrow max(S^\ell)$ (i.e. $S$ has its $minf$). However, $\{a,b\}$ has not its $msup$. Indeed, $\{a,b\}^u = \{c_i \mid i \in \mathbb{N}\}$, however, $min(\{c_i \mid i \in \mathbb{N}\}) = \emptyset$. It follows that, $\{a,b\}^u \neq \uparrow min(\{c_i \mid i \in \mathbb{N}\})$ that is $\{a,b\}$ has not its $msup$.

\begin{figure}[b]
\centering
\begin{minipage}{0.16\linewidth} 
\centering
\scalebox{.72}{\input{figures/completemeetmultilattice.tex}}
\caption{A complete meet-semimultilattice that is not a join-semimultilattice\label{fig:problemincompletemsupminf}}
\end{minipage}
\hfill
\begin{minipage}{0.8\linewidth} 
\centering
\scalebox{.7}{\input{figures/twonotimplythreemultimeet.tex}}
\caption{For all $x,y$ in this poset, $\{x,y\}$ has its $minf$. That is, this poset is a multistructure following \cite{benado1955ensembles} but not a multilattice following \cite{cordero2004new} (see definition \ref{def:multilattice}) \label{fig:twonotimplythreeinmultilattices}}
\end{minipage}
\end{figure}

\subsection{Two does not imply Three}
When \cite{benado1955ensembles} introduced the notion of multilattices (or multistructures), he considered only set of two elements, (i.e. a multilattice following \cite{benado1955ensembles} is a poset such that for all $x,y \subseteq P$, the set $\{x,y\}$ has its $msup$ and its $minf$). However, unlike lattices, this property is not sufficient to have the multilattice defined here (i.e. having a $msup$ and a $minf$ for all non empty finite subsets). This fact was underlined by \cite{benado1955ensembles} himself when he showed that from the algebraic point of view, the $msup$ and $minf$ operators are not associative as it is the case of the $sup$ and $inf$ in lattices. Figure \ref{fig:twonotimplythreeinmultilattices} shows the Hasse diagram of a poset $(P, \leq)$ s.t. $(\forall i, j \in \mathbb{N})$ $abc_i \leq abc_{i+1}$, $abc_{i} \leq ab_{j}$ , $abc_{i} \leq ac_{j}$, $abc_{i} \leq bc_{j}$, $ab_{j} \leq a$, $ab_{j} \leq b$, $ac_{j} \leq a$, , $ac_{j} \leq c$, $bc_{j} \leq b$ and $bc_{j} \leq c$.  

All pair of objects have their $msup$ and $minf$ but it is still not a multilattice. For instance, the set $\{a,b,c\}$ has not its $minf$. Indeed, $\{a,b,c\}^\ell = \{abc_i \mid i \in \mathbb{N}\}$, however, $max(\{a,b,c\}^\ell) = \emptyset$. It follows that, $\{a,b,c\}^\ell \neq \downarrow max(\{a,b,c\}^\ell)$ that is $\{a,b,c\}$ has not its $minf$.  


==> sections/proofs.tex <==
\section{Appendix - Proofs\label{appendix:proofs}}

\subsection{Proof of lemma \ref{lemma:propertiesminandarrows}}
\input{proofs/proof1.tex}

\subsection{Proof of lemma~\ref{lemma:lowerboundsarestables}}
\input{proofs/proof2.tex}

\subsection{Proof of lemma \ref{lemma:propertiesarrowsandembeddings}}
\input{proofs/proof21.tex}

\subsection{Proof of lemma \ref{lemma:downandupclosure}}
\input{proofs/proof3.tex}

%\subsection{Proof of lemma \ref{lemma:closureSystemAndMeetStructure}}
%\input{proofs/proof4.tex}

\subsection{Proof of Proposition \ref{prop:orderreversingmappints}} 
\input{proofs/proof5.tex}

\subsection{Proof of Proposition \ref{prop:compositionbetweenextandcov}} 
\input{proofs/proof6.tex}

\subsection{Proof of Theorem \ref{thm:representational}}
\input{proofs/proof7.tex}

\subsection{Proof of Proposition \ref{prop:setsystemisaextentset}}
\input{proofs/proof8.tex}



\subsection{Proof of Proposition \ref{prop:extintclosure}}
\input{proofs/proof9.tex}


\subsection{Proof of Theorem \ref{thm:upperboundedmeetsemiolattice}}
\input{proofs/proof10.tex}


\subsection{Proof of Proposition \ref{prop:alliscoverable}}
\input{proofs/proof11.tex}



\subsection{Proof or Proposition \ref{prop:support-closed-and-maximal-common}}
\input{proofs/proof12.tex}





\subsection{Proof of Theorem \ref{thm:chaincompletetoMultilattices}}
\input{proofs/proof13.tex}



\subsection{Proof of Theorem \ref{thm:computingUpperApproximations}}
\input{proofs/proof14.tex}


\subsection{Proof of Theorem \ref{thm:allinformationisinsupportclosed}}
\input{proofs/proof15.tex}


\subsection{Proof of Theorem \ref{thm:upperboundedmeetsemihyperlattice}}
\input{proofs/proof16.tex}

\subsection{Proof of Proposition \ref{prop:problemWithPextInPatternMultistructure}} 
\input{proofs/proof17.tex}

\subsection{Proof of Proposition \ref{prop:antichaintomultilattices}}
\input{proofs/proof18.tex}

\subsection{Proof of Theorem \ref{thm:antichaincompletion}}
\input{proofs/proof19.tex}

\subsection{Proof of Theorem \ref{thm:directCompletion}}
\input{proofs/proof20.tex}
